A Next Basket Recommendation Reality Check

The goal of a next basket recommendation (NBR) system is to recommend items for the next basket for a user, based on the sequence of their prior baskets. Recently, a number of methods with complex modules have been proposed that claim state-of-the-art performance. They rarely look into the predicted basket and just provide intuitive reasons for the observed improvements, e.g., better representation, capturing intentions or relations, etc. We provide a novel angle on the evaluation of next basket recommendation methods, centered on the distinction between repetition and exploration: the next basket is typically composed of previously consumed items (i.e., repeat items) and new items (i.e, explore items). We propose a set of metrics that measure the repeat/explore ratio and performance of NBR models. Using these new metrics, we analyze state-of-the-art NBR models. The results of our analysis help to clarify the extent of the actual progress achieved by existing NBR methods as well as the underlying reasons for the improvements. Overall, our work sheds light on the evaluation problem of NBR and provides useful insights into the model design for this task.

==> sections/__latexindent_temp.tex <==
% !TEX root = ../main.tex

\section{Introduction}

Over the years, \ac{NBR} has received a considerable amount of interest from the research community \citep{fpmc,dream,bai2018attribute}. Baskets, or sets of items that are purchased or consumed together, are pervasive in many real-world services, with e-commerce and grocery shopping as prominent examples~\citep{hao, raeder}. 
Given a sequence of baskets that a user has purchased or consumed in the past, the goal of a \ac{NBR} system is to generate the next basket of items that the user would like to purchase or consume next. 
Within a basket, items have no temporal order and are equally important. 
A key difference between \ac{NBR} and session-based or sequential item recommendations is that \ac{NBR} systems need to deal with multiple simultaneous items in one set. 
Therefore, models designed for item-based recommendation are not fit for basket-based recommendation, and dedicated \ac{NBR} methods have been proposed~\citep{sets2sets, sun2020timestamp2}. 

Numerous deep learning techniques have been developed to address sequential item recommendation problems, building on the well-documented capacity of neural methods to capture hidden relations and automatically learn representations~\citep{batmaz-2019-deep}. 
Against this background, recent years have witnessed many proposals to address different aspects of the \ac{NBR} task with neural methods, e.g., item-to-item relations~\cite{beacon}, cross-basket relations~\cite{dnntsp}, noise within a basket~\cite{clea}. 
%We could expect that more fancy modules with ``reasonable'' hypotheses will be proposed, which will make the \ac{NBR} model even more complex~\mozh{The last sentence is not very clear.}. 

Recent analyses have shown that neural-based approaches might not be the best approaches for recommendation yet \cite{notwinning}.
In sequential recommendation problems, we see that shows that such methods may be outperformed by simple nearest neighbor or graph-based baselines~\cite{realprogress}. 
This also holds for simple recommendation, where linear models and neighbor-based approaches are still overperforming complex methods \cite{dacrema2021troubling}.

In this paper, we perform a similar analysis for the \acl{NBR} task (instead of the generic sequential recommendation problem).
We notice that the same factors that account for the phenomena observed by \citet{realprogress} are also featured in recent research on the \acl{NBR} task. 
These issues seem to stem from an overall reproducibility problem in the recommendation literature \cite{dacrema2021troubling,notwinning, realprogress}.
This includes weak or missing baselines, the use of different datasets in different papers, and of non-standard metrics. 
For example, some methods \cite{dream, bai2018attribute, beacon, clea, intnet} only compare with previous (deep) learning-based methods and avoid comparing with a simple Personal-TopFreq baseline, which recommends the most $k$ frequent items in the users’ historical records as the next basket. 
Many recent publications \cite{recency, tifuknn, dnntsp, clea} do not compare with each other. And in~\cite{clea}, sampled metrics \cite{sasrec} are used to evaluate the performance even though this is not encouraged~\cite{sampledmetrics}.
%~\mozh{because}.
Finally, previous studies on models for \ac{NBR} tend to use limited case studies and ablation studies to demonstrate the effectiveness of their proposed methods. 
They forego a deeper analysis of what items are actually recommended in the next basket.

\sami{We might miss a bit of context here. Why is looking into what items are recommended important?}
%and only use conventional item recommendation and ranking metrics, such as recall, nDCG, or personal hit ratio.

Given the state of affairs sketched above, we believe that it is important to perform a reality check on current \ac{NBR} methods, in order to find out how much progress we have actually made and whether a specific proposed module is responsible for the observed improvements.
We propose a novel \emph{repetition and exploration} perspective to evaluate \acl{NBR} methods. Baskets recommended in a \ac{NBR} scenario consist of \emph{repeat items} (items that the user consumed before, in previous baskets) and \emph{explore items} (items that are new to the user).
In order to improve our understanding of the relative performance of \ac{NBR} models, especially regarding repeat items and explore items, we introduce a set of task-specific metrics for \ac{NBR}.
Those metrics help us to understand what type of items are present in the recommended basket and assess the performance of models when proposing new items vs.\  already-purchased items. 
%At the same time, we propose a new simple baseline GP-Freq, since the comparison with P-TopFreq is somewhat ``unfair'' due to the usage of basket slots. \mozh{The last sentence is not clear. What are basket slots?}

With the proposed metrics for \ac{NBR} and a new baseline, GP-Freq, we evaluate the performance of state-of-the-art \ac{NBR} models on three benchmark datasets, with different repeat-explore patterns. 
We arrive at several important findings:
\begin{enumerate*}[label=(\arabic*)]
\item No \ac{NBR} method can consistently outperform all other methods across different datasets. 
\item All published methods are heavily skewed to either repetition or exploration compared to the ground-truth, which might harm long-term engagement. 
\item There is a large performance gap between repetition and exploration; repeat item recommendation is much more easier. 
\item Several deep learning-based neural methods are inferior to simple frequency baselines P-TopFreq and GP-TopFreq in many settings. 
\item Being biased towards repetition and its improvements in repetition accounts for most of the performance gains of recently published methods, even though many complex modules or strategies specifically target explore items. 
\item GP-TopFreq is a highly competitive baseline across different datasets, and comparing to it, observed improvements of several state-of-the-art methods are limited.
\end{enumerate*}

Overall, our work sheds light on the state-of-the-art of \ac{NBR}, provides suggestions to revise the metrics of \ac{NBR} evaluation,  helps to understand the current progress and the underlying reasons for improvements, and provides further insights for the design of \ac{NBR} models. 

